FIPAC: Thwarting Fault- and Software-Induced Control-Flow Attacks with ARM Pointer Authentication

With the improvements of computing technology, more and more applications embed powerful ARM processors into their devices. These systems can be attacked by redirecting the control-flow of a program to bypass critical pieces of code such as privilege checks or signature verifications. Control-flow hijacks can be performed using classical software vulnerabilities, physical fault attacks, or software-induced fault attacks. To cope with this threat and to protect the control-flow, dedicated countermeasures are needed. To counteract control-flow hijacks, control-flow integrity~(CFI) aims to be a generic solution. However, software-based CFI typically either protects against software or fault attacks, but not against both. While hardware-assisted CFI can mitigate both types of attacks, they require extensive hardware modifications. As hardware changes are unrealistic for existing ARM architectures, a wide range of systems remains unprotected and vulnerable to control-flow attacks. In this work, we present FIPAC, an efficient software-based CFI scheme protecting the execution at basic block granularity of ARM-based devices against software and fault attacks. FIPAC exploits ARM pointer authentication of ARMv8.6-A to implement a cryptographically signed control-flow graph. We cryptographically link the correct sequence of executed basic blocks to enforce CFI at this granularity. We use an LLVM-based toolchain to automatically instrument programs. The evaluation on SPEC2017 with different security policies shows a code overhead between 54-97\% and a runtime overhead between 35-105%. While these overheads are higher than for countermeasures against software attacks, FIPAC outperforms related work protecting the control-flow against fault attacks. FIPAC is an efficient solution to provide protection against software- and fault-based CFI attacks on basic block level on modern ARM devices.

==> settings.tches.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2569-2925}
\makeatletter
\setDOI{10.13154/tches.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

\setkeys{IACR}{journal=tches}

